A triplet of the only pulsation mode detected in the DAV star G132-12

Hydrogen atmosphere pulsating white dwarfs, also known as DAV stars, are the most abundant type of pulsating white dwarfs. High-temperature DAV stars exhibit in general a small number of pulsation modes and stable frequencies. G132-12 is one of the pulsating hydrogen atmosphere white dwarf stars which lies close to the blue edge of the instability strip. Previous researches reported that G132-12 might have only one pulsation mode with the period of 212.69 s. To study the pulsation properties of G132-12 in detail, we carried out a bi-site observation campaign in October 2019. Time series photometric data were collected during around 154 hours in total. A Fourier Analysis reveals 3 frequencies which are identified as the triplet of a $l = 1$ g-mode pulsation with the period of 212.499 s. The rotational period is derived as $P_{rot} = 35.0\pm6.7$ hours and the inclination of the rotational axis to the line of sight is $70^{\circ}$. G132-12 could be an ideal target for measuring the cooling scale of this white dwarf star with only one excited pulsation mode detected.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

